Design Automation for Efficient Deep Learning Computing

Efficient deep learning computing requires algorithm and hardware co-design to enable specialization: we usually need to change the algorithm to reduce memory footprint and improve energy efficiency. However, the extra degree of freedom from the algorithm makes the design space much larger: it's not only about designing the hardware but also about how to tweak the algorithm to best fit the hardware. Human engineers can hardly exhaust the design space by heuristics. It's labor consuming and sub-optimal. We propose design automation techniques for efficient neural networks. We investigate automatically designing specialized fast models, auto channel pruning, and auto mixed-precision quantization. We demonstrate such learning-based, automated design achieves superior performance and efficiency than rule-based human design. Moreover, we shorten the design cycle by 200x than previous work, so that we can afford to design specialized neural network models for different hardware platforms.

==> figures/haq/bismo_latency_v2_figures.tex <==
\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.93\linewidth]{figures/haq/bismo_v2.pdf}
    \caption{Quantization policy under latency constraints for MobileNet-V2 on BISMO. Similar to \fig{fig:bismo_v1}, depthwise layer is assigned with fewer bits on the edge accelerator, and pointwise layer is assigned with fewer bits on the cloud accelerator.}
    \label{fig:bismo_latency_v2}
\end{figure*}


==> figures/haq/bitfusion_energy_tables.tex <==
\begin{table}[!t]
    \renewcommand*{\arraystretch}{1.15}
    \setlength{\tabcolsep}{4pt}
    \small\centering
    \begin{tabular}{lccccc} 
        \toprule
        & Weights & Activations & Acc.-1 & Acc.-5 & Energy \\
        \midrule
        PACT~\cite{Choi:2018uw} & 4 bits & 4 bits & 62.44 & 84.19 & 13.47 mJ \\
        Ours & \emph{flexible} & \emph{flexible} & \textbf{64.78} & \textbf{85.85} & 13.69 mJ \\
        \midrule
        PACT~\cite{Choi:2018uw} & 6 bits & 4 bits & 67.51 & 87.84 & 16.57 mJ \\
        Ours & \emph{flexible} & \emph{flexible} & \cellcolor{red!15}\textbf{70.37} & \cellcolor{red!15}\textbf{89.40} & \cellcolor{red!15}16.30 mJ \\
        \midrule
        PACT~\cite{Choi:2018uw} & 6 bits & 6 bits & 70.46 & 89.59 & 26.80 mJ \\
        Ours & \emph{flexible} & \emph{flexible} & \textbf{70.90} & \textbf{89.73} & 26.67 mJ \\
        \midrule
        Original & 8 bits & 8 bits & \cellcolor{red!15}70.82 & \cellcolor{red!15}89.95 & \cellcolor{red!15}31.03 mJ \\
        \bottomrule
    \end{tabular}
    \caption{Energy-constrained quantization on BitFusion (MobileNet-V1 on ImageNet). Our framework reduces the power consumption by \textbf{2$\times$} with nearly no loss of accuracy compared with the fixed bitwidth quantization.}
    \label{tbl:bitfusion_energy}
\end{table}

==> figures/haq/bitfusion_latency_tables.tex <==
\begin{table}[!t]
    \renewcommand*{\arraystretch}{1.15}
    \setlength{\tabcolsep}{4pt}
    \small\centering
    \begin{tabular}{lccccc}
        \toprule
        & Weights & Activations & Acc.-1 & Acc.-5 & Latency \\
        \midrule
        PACT~\cite{Choi:2018uw} & 4 bits & 4 bits & 62.44 & 84.19 & 7.86 ms \\
        Ours & \emph{flexible} & \emph{flexible} & \textbf{67.45} & \textbf{87.85} & 7.86 ms \\
        \midrule
        PACT~\cite{Choi:2018uw} & 6 bits & 4 bits & 67.51 & 87.84 & 11.10 ms \\
        Ours & \emph{flexible} & \emph{flexible} & \cellcolor{red!15}\textbf{70.40} & \cellcolor{red!15}\textbf{89.69} & \cellcolor{red!15}11.09 ms \\
        \midrule
        PACT~\cite{Choi:2018uw} & 6 bits & 6 bits & 70.46 & 89.59 & 19.99 ms \\
        Ours & \emph{flexible} & \emph{flexible} & \textbf{70.90} & \textbf{89.95} & 19.98 ms \\
        \midrule
        Original & 8 bits & 8 bits & \cellcolor{red!15}70.82 & \cellcolor{red!15}89.85 & \cellcolor{red!15}20.08 ms \\
        \bottomrule
    \end{tabular}
    \caption{Latency-constrained quantization on BitFusion (MobileNet-V1 on ImageNet). Our framework can reduce the latency by \textbf{2$\times$} with almost no loss of accuracy compared with the fixed bitwidth (8 bits) quantization.}
    \label{tbl:bitfusion_latency}
\end{table}

==> figures/haq/edge_cloud_datasheet.tex <==
\begin{table}[t]
    \renewcommand*{\arraystretch}{1.15}
    \setlength{\tabcolsep}{4pt}
    \small\centering
    \begin{tabular}{lcccccc} 
        \toprule
        & Hardware & Batch & PE Array & AXI port & Block RAM \\
        \midrule
        Edge & Zynq-7020 & 1 & 8$\times$8 & 4$\times$64b & 140$\times$36Kb \\
        Cloud & VU9P & 16 & 16$\times$16 & 4$\times$256b & 2160$\times$36Kb \\
        \bottomrule
    \end{tabular}
    \caption{The configurations of edge and cloud accelerators.}
    \label{tbl:edge_cloud}
\end{table}


==> figures/haq/model_size_figures.tex <==


\begin{figure*}[!t]
    \centering
    \includegraphics[width=\linewidth]{figures/haq/model_size}
    \caption{Quantization policy under model size constraints for MobileNet-V2. Our RL agent allocates \emph{more} bits to the depthwise convolutions, since depthwise convolutions have \emph{fewer} number of parameters.}
    \label{fig:model_size}
\end{figure*}

==> figures/haq/model_size_tables.tex <==
\begin{table*}[!t]
    \renewcommand*{\arraystretch}{1.15}
    \small\centering
    \begin{tabular}{lcccccccccccc} 
        \toprule
        & & \multicolumn{3}{c}{MobileNet-V1} & \multicolumn{3}{c}{MobileNet-V2} & \multicolumn{3}{c}{ResNet-50} \\
        \cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}
        & Weights & Acc.-1 & Acc.-5 & Model Size & Acc.-1 & Acc.-5 & Model Size & Acc.-1 & Acc.-5 & Model Size \\
        \midrule
        Han~\etal~\cite{han2015deep} & 2 bits & 37.62 & 64.31 & 1.09 MB & 58.07 & 81.24 & 0.96 MB & 68.95 & 88.68 & 6.32 MB \\
        Ours & \emph{flexible} & \textbf{57.14} & \textbf{81.87} & 1.09 MB & \textbf{66.75} & \textbf{87.32} & 0.95 MB & \textbf{70.63} & \textbf{89.93} & 6.30 MB \\
        \midrule
        Han~\etal~\cite{han2015deep} & 3 bits & 65.93 & 86.85 & 1.60 MB & 68.00 & 87.96 & 1.38 MB & 75.10 & 92.33 & 9.36 MB \\
        Ours & \emph{flexible} & \textbf{67.66} & \textbf{88.21} & 1.58 MB & \textbf{70.90} & \textbf{89.76} & 1.38 MB & \textbf{75.30} & \textbf{92.45} & 9.22 MB \\
        \midrule
        Han~\etal~\cite{han2015deep} & 4 bits  & 71.14 & 89.84 & 2.10 MB & 71.24 & 89.93 & 1.79 MB & \textbf{76.15} & 92.88 & 12.40 MB \\
        Ours & \emph{flexible} & \textbf{71.74} & \textbf{90.36} & 2.07 MB & \textbf{71.47} & \textbf{90.23} & 1.79 MB & 76.14 & \textbf{92.89} & 12.14 MB \\
        \midrule
        Original & 32 bits & 70.90 & 89.90 & 16.14 MB & 71.87 & 90.32 & 13.37 MB & 76.15 & 92.86 & 97.49 MB \\
        \bottomrule
    \end{tabular}
    \caption{Model size-constrained quantization on ImageNet. Compared with Deep Compression~\cite{Han:2017td}, our framework achieves higher accuracy under similar model size (especially under high compression ratio).}
    \label{tbl:model_size}
\end{table*}

==> figures/haq/overview.tex <==
\def\model{\textbf{H}ardware-Aware \textbf{A}utomated \textbf{Q}uantization\xspace}
\def\modelshort{HAQ\xspace}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.93\textwidth]{figures/haq/overview.pdf}
    \caption{An overview of our \model (\modelshort) framework. We leverage the reinforcement learning to automatically search over the huge quantization design space with hardware in the loop. The agent propose an optimal bitwidth allocation policy given the amount of computation resources (\ie, latency, power, and model size). Our RL agent integrates the hardware accelerator into the exploration loop so that it can obtain the direct feedback from the hardware, instead of relying on indirect proxy signals.}
    \label{fig:haq_overview}
\end{figure*}

==> figures/haq/teaser_figures.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{figures/haq/teaser.pdf}
    \caption{We need \textbf{mixed precision} for different layers. We quantize MobileNets~\cite{howard2017mobilenets} to different number of bits (both weights and activations), and it lies on a better pareto curve (yellow) than fixed bit quantization (blue). The reason is that different layers have different redundancy and have different arithmetic intensity (OPs/byte) on the hardware, which advocates for using mixed precision for different layers.}
    \label{fig:teaser}
\end{figure}

